Quantum Conformal Prediction for Reliable Uncertainty Quantification in Quantum Machine Learning

In this work, we aim at augmenting the decisions output by quantum models with "error bars" that provide finite-sample coverage guarantees. Quantum models implement implicit probabilistic predictors that produce multiple random decisions for each input through measurement shots. Randomness arises not only from the inherent stochasticity of quantum measurements, but also from quantum gate noise and quantum measurement noise caused by noisy hardware. Furthermore, quantum noise may be correlated across shots and it may present drifts in time. This paper proposes to leverage such randomness to define prediction sets for both classification and regression that provably capture the uncertainty of the model. The approach builds on probabilistic conformal prediction (PCP), while accounting for the unique features of quantum models. Among the key technical innovations, we introduce a new general class of non-conformity scores that address the presence of quantum noise, including possible drifts. Experimental results, using both simulators and current quantum computers, confirm the theoretical calibration guarantees of the proposed framework.

==> Sections/1_Intro.tex <==
\section{Introduction}
\label{sec:intro}
%\PARstart{T}{his}
Quantum machine learning  is currently viewed as a promising paradigm for the optimization of algorithms that can leverage existing noisy intermediate scale quantum (NISQ) computers \cite{biamonte2017quantum,schuld2021machine, simeone2022introduction}. As for classical machine learning, the principle underlying quantum machine learning is \emph{generalization}: While the optimization is based on a limited training set, the designer targets the performance of the algorithm \emph{outside} the training set, under testing conditions that are statistically similar --  ideally equivalent -- to those encountered during training data collection. The central technical challenge is therefore that of understanding and controlling accuracy and uncertainty levels for decisions taken by a trained algorithm on test data  \cite{shalev2014understanding,simeone2022machine}. 

As we will summarize in the next subsection, most work on the subject of generalization for quantum machine learning has focused on studying scaling laws on the amount of data required to ensure desired performance levels on test data (see, e.g., \cite{caro2022generalization}). In contrast, this article introduces a novel \emph{operational} framework for the derivation of practically relevant generalization guarantees.  The approach, referred to as \emph{quantum conformal prediction} (QCP), applies a post-hoc calibration step based on held-out calibration, or validation, data to pre-trained quantum machine learning models. QCP builds on \emph{conformal prediction} (CP), a general calibration methodology that is currently experiencing renewed attention in the area of classical machine learning \cite{vovk2022algorithmic,tibshirani2019conformal, barber2021predictive, angelopoulos2021gentle}. Unlike classical CP, QCP takes into account the unique nature of quantum models as \emph{probabilistic} machines, due to the inherent randomness of quantum measurements \cite{simeone2022introduction, cai2022quantum}. 


\begin{figure}
  \centering
  \includegraphics[width=0.65\textwidth]{Figs/overall.pdf}
  \caption{Comparison between (\emph{i}) quantum generalization analysis \cite{caro2022generalization,banchi2021generalization, jose2022transfer, abbas2021power, weber2022toward} and (\emph{ii}) quantum conformal prediction (QCP), which is introduced in this work. Quantum generalization analysis provides \emph{analytical} bounds on the generalization error that explicitly capture the general dependence on the number of training examples (typically assuming an infinite number of shots). Based on such bounds, one is able to conclude that, if the number of data points scales sufficiently quickly with respect to the model complexity, the trained model generalizes well outside the training data. In contrast, QCP provides an \emph{operational} way of quantifying the uncertainty of the decisions made outside the training set (shaded areas). The resulting ``error bars'' are  \emph{guaranteed} to contain the ground-truth output with a desired probability, regardless of the amount of data, of the number of measurements, of the ansatz of the quantum machine learning model, of the training algorithm, and of the presence of quantum hardware noise. (\emph{iii}) As an illustration of the results that can be obtained via generalization analysis, this panel shows the generalization bounds derived in \cite{caro2022generalization} as a function of number of training examples for different numbers $T$ of trainable local quantum gates (see Appendix~\ref{appendix:gen_bounds} for details). As suggested by the plot, while very useful to identify general trends and scaling laws, generalization analyses only provide numerically meaningful bounds with a very large number of training examples. \label{fig:overall}}
\end{figure}

\subsection{Generalization Analysis vs. Conformal Prediction}

As illustrated in Fig. \ref{fig:overall}, \emph{generalization analysis} focuses on the identification of \emph{analytical} scaling laws on the amount of data required to ensure desired performance levels on test data \cite{shalev2014understanding}, possibly as a function of the training algorithm \cite{mcallester1999pac, guedj2019primer} and of the data distribution \cite{russo2016controlling, xu2017information} (see also \cite{simeone2022machine}). Related studies have also been initiated for quantum machine learning, with recent results including \cite{caro2022generalization,banchi2021generalization, jose2022transfer, abbas2021power, weber2022toward}. 


As a notable example, reference \cite{caro2022generalization} reveals the important insight that the \emph{generalization error}, i.e., the discrepancy between training and test losses, for quantum models grows as the square root of the number of gates $T$ and with the inverse of the square root of the size of the data set. While critical to gauge the feasibility to train quantum circuits, such results provide limited \emph{operational} guidelines concerning the uncertainty associated with decisions made on test data when training data are limited (see Fig.~\ref{fig:overall} and Appendix~\ref{appendix:gen_bounds} for details). 




Most papers on quantum machine learning, including on generalization analyses, treat the output of a quantum model as \emph{deterministic}, implicitly assuming that expected values of observables can be calculated exactly \cite{caro2022generalization,banchi2021generalization, jose2022transfer, abbas2021power, weber2022toward}. In practice, for this to be an accurate modelling assumption, one needs to carry out a sufficiently large -- strictly speaking, infinite -- number of measurements, or \emph{shots}, at the output of the quantum circuit (see Fig.~\ref{fig:overall}, left column). These measurements are averaged to obtain the final prediction. From a statistical viewpoint, this assumption conveniently makes a quantum  models \emph{likelihood-based}, in the sense that one can evaluate exactly the probability of any output given an input and the model parameters (see, e.g., \cite{simeone2022machine}). 

In practice, however, quantum models are more properly described as being \emph{implicit}, or \emph{simulation-based}, in the sense that they only provide random samples from a given, inaccessible, likelihood \cite{duffield2022bayesian}. The generalization capabilities of \emph{generative} quantum models -- an example of implicit models -- have been recently studied in a separate line of research, including in  \cite{du2022theory, gili2022evaluating}. 


In contrast to generalization analysis, CP \cite{vovk2022algorithmic} does not aim at obtaining analytical conclusions concerning sample efficiency. Rather, it provides a  general methodology to obtain ``error bars'' with formal guarantees on the probability of covering the correct test output. Such guarantees hold irrespective of the size of the training data set \cite{vovk2022algorithmic, barber2021predictive}. We will specifically focus here on \emph{split}, or \emph{validation-based}, CP \cite{vovk2022algorithmic}. 

Validation-based CP is a  post-hoc \emph{calibration} methodology that applies to \emph{pre-trained} machine learning models. It produces set predictors, such as intervals for regression problems, that are provably guaranteed to contain the true target with probability no smaller than the predetermined coverage level (see Fig. \ref{fig:overall}, right column). This goal is accomplished by utilizing a \emph{calibration data set}, and is formalized in terms of probabilities with respect to the random generation of testing and calibration data. 

To the best of our knowledge, as we further discuss next, this is the first work that proposes to leverage CP for the purpose of reliably quantifying uncertainty for quantum machine learning models.

\subsection{Quantum Conformal Prediction}
\label{subsec:intro_qcp}
The goal of the proposed framework, referred to as QCP, is to assign \emph{well-calibrated} ``error bars'' to the decisions made by the quantum machine learning models. The ``error-bars'' are formally subsets of the output space, and \emph{calibration} refers to the property of containing the true target with probability no smaller than a predetermined \emph{coverage} level. Importantly, with QCP, calibration holds irrespective of the number of training data set, of the ansatz of the quantum machine learning model, of the training algorithm, of the number of shots, and of the presence of  quantum hardware noise \cite{cai2022quantum}. The only assumption required for QCP is the \emph{finite exchangeability} of calibration data and test data, which is practically satisfied under the conventional independent and identically distributed (i.i.d.) assumption \cite{vovk2022algorithmic}. We refer to Fig.~\ref{fig:conven_CP_cartoon}, left bar, for an illustration of the properties of QCP. 

An important challenge in applying CP to quantum machine learning models is that conventional CP targets  \emph{deterministic}, likelihood-based, models that produce point predictions, such as conventional neural networks, while quantum models are inherently \emph{stochastic}, or sampling-based. Recent work \cite{wang2022probabilistic} introduced a novel CP scheme, referred to as \emph{probabilistic CP} (PCP), that applies to \emph{classical} sampling-based  predictors. The main motivation of reference \cite{wang2022probabilistic} in leveraging probabilistic outputs is to address a mismatch between the assumed probabilistic model and the ground-truth distribution, which may require disconnected predictive sets (see \cite[Fig. 1]{wang2022probabilistic}, as well as Fig.~\ref{fig:pcp_scoring} for a preview). QCP is inspired by reference \cite{wang2022probabilistic}, although our motivation stems from the fact that quantum models are \emph{inherently} implicit probabilistic models. {\color{black} The proposed method is aligned with the framework in \cite{deville2021new} in that it operates with any finite number of copies of a quantum state, not requiring the exact evaluation of an expected value. }

Our main contributions are as follows:
\begin{itemize}
    \item We introduce QCP, a post-hoc calibration methodology for quantum machine learning models that produces predictive sets with controllable guarantees on the generalization performance.
    \item To keep the article self-contained, we provide an introduction to classical CP and PCP. 
    \item We present, for reference, a direct application of CP to conventional deterministic and likelihood-based quantum machine learning that assume the use of an infinite number of shots.
    \item We detail experimental results based on both simulation and quantum hardware implementation. The experiments bring evidence on the merits of QCP, confirming its theoretical calibration guarantees.
    \item Among our main conclusions, we show that, when quantum models are augmented with QCP, it is generally advantageous not to average over the shots, as typically done in the literature. Rather, treating the shots as separate samples allows QCP to obtain more informative error bars.
\end{itemize}




The rest of the article is organized as follows. In Sec. \ref{sec:CCP}, conventional CP for classical deterministic models is reviewed, and a direct application of CP  to quantum machine learning models is presented that assumes an infinite number of shots. Sec. \ref{sec:probabilistic_CP}  describes PCP for classical probabilistic models as proposed in \cite{wang2022probabilistic}. Then,  QCP for quantum machine learning models is introduced in Sec. \ref{sec:QCP}, with Sec. \ref{sec:finite_number_guarantee} addressing the aspect of performance evaluation.  Numerical and experimental settings are provided in Sec.~\ref{sec:experimental_settings}, with results presented in  Sec.~\ref{sec:experimental_results}. Sec.~\ref{sec:conclusion} concludes the article.    



==> Sections/2_CP.tex <==
\section{Conformal Prediction for Deterministic Models}
\label{sec:CCP}
In this section, we first review conventional CP, which applies a post-hoc calibration step to \emph{deterministic} predictive models \cite{vovk2022algorithmic}. Then, we introduce a direct application of this approach to quantum models, and we highlight its limitations. This discussion will motivate the proposed QCP method, which is presented in Sec.~\ref{sec:QCP}.


\subsection{Calibrating Deterministic Predictors via Set Prediction}
\label{sec:classical_CP}
Consider a class of classical parametric predictors $f(\cdot|\theta)$ with parameter vector $\theta$. The predictor produces an output $y\in\mathcal{Y}$ given an input $x\in\mathcal{X}$ as
\begin{align}
    \hat{y} = f(x|\theta).
\end{align}
The domains $\mathcal{X}$ and $\mathcal{Y}$ of input and output, respectively, can be either discrete or continuous depending on the problem of interest. The parameter vector $\theta$ is optimized using a \emph{training data set} \begin{align} \mathcal{D}^\text{tr} = \{ z^\text{tr}[i]=(x^\text{tr}[i],y^\text{tr}[i]) \}_{i=1}^{|\mathcal{D}^\text{tr}|}\end{align}  via an arbitrary training algorithm that returns a parameter vector $\theta_{\mathcal{D}^\text{tr}}$ and a corresponding predictor $\hat{y} = f(x|\theta_{\mathcal{D}^\text{tr}})$. 

As we detail in the next subsection, CP is a post-hoc calibration scheme that processes the prediction $\hat{y}$ by using a \emph{calibration data set} \begin{align}\mathcal{D}^\text{cal} = \{ z[i]=(x[i],y[i]) \}_{i=1}^{|\mathcal{D}^\text{cal}|}\end{align} to obtain a \emph{well-calibrated} set prediction. Given a test input $x$, a \emph{set predictor} $\Gamma(x|\mathcal{D}^\text{cal},\theta) \subseteq \mathcal{Y}$ returns a subset of the possible output values in set $\mathcal{Y}$. The set $\Gamma(x|\mathcal{D}^\text{cal},\theta)$ is said to be \emph{well calibrated} if it contains the true target $y$ with probability no smaller than a predetermined \emph{coverage level} $1-\alpha$.


\begin{figure*}
  \centering
  \includegraphics[width=0.88\textwidth]{Figs/conven_CP_cartoon.png}
  \caption{Illustration of conventional CP for deterministic (likelihood-based) models: (\emph{i}) Based on any trained model parameter vector  $\theta_{\mathcal{D}^\text{tr}}$ and given a scoring function $s(\cdot|\theta_{\mathcal{D}^\text{tr}})$, e.g., the quadratic loss, CP first computes scores for every calibration example in an offline phase; (\emph{ii}) Based on the  $|\mathcal{D}^\text{cal}|$ calibration scores, CP divides the real line into an acceptance region and a rejection region by computing the $(1-\alpha)$-quantile of the calibration scores; (\emph{iii}) CP constructs a set predictor for a test input $x$ by collecting all  candidate outputs $y' \in \mathcal{Y}$ whose scores lie in the acceptance region; (\emph{iv}) The obtained CP set predictor (green circle) is guaranteed to satisfy the validity condition \eqref{eq:validity}.}
  \label{fig:conven_CP_cartoon}
\end{figure*}



To formalize the notion of calibration for set predictors, let us make the mild assumption that the calibration examples $z[i]=(x[i], y[i])$ for $i=1,...,|\mathcal{D}^\text{cal}|$ in set $\mathcal{D}^\text{cal}$, along with the test example $z=(x,y)$, are (finitely) exchangeable random variables. As a point of notation, observe that we use bold fonts to denote random variables.
\begin{assumption}[Finite exchangeability \protect{\cite[Sec.~II]{caves2002unknown}}]\label{assum:classical} Calibration data set $\mathbfcal{D}^\text{cal}$ and a test data point $\mathbf{z}$ are finitely exchangeable random variables, i.e., the joint distribution $p(\mathcal{D}^\text{cal},z) = p(z[1],...,z[|\mathcal{D}^\text{cal}|],z)$ is invariant to any permutation of the variables $\{ \mathbf{z}[1],...,\mathbf{z}[|\mathcal{D}^\text{cal}|],\mathbf{z} \}$. Mathematically, we have the equality $p(z[1],...,z[|\mathcal{D}^\text{cal}|+1]) = p(z[\pi(1)],...,z[\pi(|\mathcal{D}^\text{cal}|+1)])$ with $z=z[|\mathcal{D}^\text{cal}|+1]$, for any permutation operator $\pi(\cdot)$. Note that the standard assumption of i.i.d. random variables satisfies finite exchangeability.
\end{assumption}
It is important to emphasize that only exchangeability of calibration and test data is assumed (Assumption~\ref{assum:classical}), while no requirements are imposed on the training data set $\mathcal{D}^\text{tr}$, or on the accuracy of the trained  model parameter vector $\theta_{\mathcal{D}^\text{tr}}$.
   
Given a trained model parameter vector $\theta_{\mathcal{D}^\text{tr}}$,  a set predictor ${\Gamma}(\mathbf{x}|\mathbfcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) $  is said to be \emph{well calibrated at the coverage level $1-\alpha$},  for some $\alpha \in (0,1)$, if the following inequality holds
\begin{align}
    \label{eq:validity}
    \Pr\big(\mathbf{y} \in {\Gamma}(\mathbf{x}|\mathbfcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) \big) \geq 1-\alpha, 
\end{align}
where the probability $\Pr(\cdot)$ is taken over the joint distribution $p(\mathcal{D}^\text{cal},z)$ of calibration data set and test data point. 



\subsection{Conformal Prediction}
\label{sec:classical_CP_procedure}
As mentioned, CP starts with a pre-trained model $\hat{y} = f(x|\theta_{\mathcal{D}^\text{tr}})$, and extracts from it a well-calibrated set predictor satisfying the condition (\ref{eq:validity}). To this end, CP relies on the specification of a \emph{scoring function} $s(\cdot|\theta_{\mathcal{D}^\text{tr}})$. The scoring function quantifies the \emph{performance loss} accrued by the trained model on the input-output pair $z=(x,y)$. Accordingly, a scoring function should  ideally increase when the error between prediction $\hat{y}$ and the true target $y$ increases \cite{vovk2022algorithmic}. 

As an example of scoring functions, one may consider the quadratic loss $s(z|\theta)=(y-f(x|\theta_{\mathcal{D}^\text{tr}}))^2$ for continuous target variables with $\mathcal{Y}=\mathbb{R}$, or the logistic loss $s(z|\theta)=\log(1+\exp(-y f(x|\theta_{\mathcal{D}^\text{tr}})))$ for binary random variables with $\mathcal{Y}=\{-1,1\}$ \cite{simeone2022machine}. 

Based on the calibration set $\mathcal{D}^\text{cal}$ and the target coverage level $1-\alpha$, as illustrated in Fig.~\ref{fig:conven_CP_cartoon},  CP divides the possible values returned by the scoring function for the trained model  $ f(x|\theta_{\mathcal{D}^\text{tr}})$ into an \emph{acceptance region} and a \emph{rejection region}. A set predictor ${\Gamma}({x}|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) $ for a test input $x$ is then obtained by including all candidate outputs $y'\in \mathcal{Y}$ whose scores $s((x,y')|\theta_{\mathcal{D}^\text{tr}})$ lie in the acceptance region for the trained predictor.

The threshold dividing the acceptance and rejection regions is obtained by examining the calibration set $|\mathcal{D}^\text{cal}|$. Specifically, in an \emph{offline} phase, the scores assigned by the pre-trained model are evaluated for all data points in the calibration set, obtaining the set of $|\mathcal{D}^\text{cal}|$ values $\{ s(z[1]|\theta_{\mathcal{D}^\text{tr}})  ,...,s(z[|\mathcal{D}^\text{cal}|]|\theta_{\mathcal{D}^\text{tr}})\}$. Then, CP chooses the threshold such that a fraction  $(1-\alpha)$ of calibration points returns a score value lower than the threshold. Intuitively, this ensures that all accepted output values also have probability no smaller than $1-\alpha$ due to the exchangeability assumption  in Assumption 1 \cite{vovk2022algorithmic}.  

More formally, let us define as $Q_{1-\alpha}( \{  s(z[i]|\theta_{\mathcal{D}^\text{tr}})  \}_{i=1}^{|\mathcal{D}^\text{cal}|} )$ the $\lceil(1-\alpha)(|\mathcal{D}^\text{cal}|+1)\rceil$-th smallest value in the set $\{ s(z[1]|\theta_{\mathcal{D}^\text{tr}})  ,...,s(z[|\mathcal{D}^\text{cal}|]|\theta_{\mathcal{D}^\text{tr}}),\infty \}$. The CP set predictor is defined as 
\begin{align}
    \label{eq:classical_CP_set_predictor}
    \Gamma(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) =&\Big\{ y' \in \mathcal{Y} \hspace{-0.1cm}\: : \hspace{-0.1cm}\: s((x,y')|\theta_{\mathcal{D}^\text{tr}}) \:\leq\:  Q_{1-\alpha} \big(\big\{ s({z}[i]|\theta_{\mathcal{D}^\text{tr}})\big\}_{i=1}^{ |\mathcal{D}^\text{cal}| } \big) \Big\}.
\end{align}
Fig.~\ref{fig:conven_CP_cartoon} provides an illustration of the overall CP process. 

As long as Assumption~\ref{assum:classical} holds, conventional CP guarantees that the set predictor \eqref{eq:classical_CP_set_predictor} is well calibrated for any trained model $\theta_{\mathcal{D}^\text{tr}}$.


\begin{theorem}[Calibration of deterministic CP \cite{vovk2022algorithmic}] Under Assumption~\ref{assum:classical}, for any miscoverage level $\alpha \in (0,1)$, for any trained model $\theta_{\mathcal{D}^{\text{tr}}}$, and for any scoring function $s(\cdot|\theta_{\mathcal{D}^\text{tr}})$, the CP set predictor \eqref{eq:classical_CP_set_predictor} satisfies the validity condition \eqref{eq:validity}, i.e., $\Pr( \mathbf{y} \in \Gamma(\mathbf{x}|\mathbfcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) ) \geq 1-\alpha$, with probability taken over the joint distribution of the test data $\mathbf{z}$ and calibration data set $\mathbfcal{D}^\text{cal}$. \label{ther:dcp}
\end{theorem}
For completeness, and in order to keep the presentation self-contained, a proof of Theorem~\ref{ther:dcp} can be found in Appendix~\ref{appendix:proofs}.




\subsection{Conventional Conformal Prediction for Quantum Models}
\label{subsec:quantum_models}
\label{subsec:CP_for_infinite_shot}
In this section, we introduce a direct application of conventional CP, as described in the previous subsection, to predictions obtained via quantum machine learning models. Throughout this article, we focus on general quantum machine learning models implemented by a \emph{parameterized quantum circuit} (PQC) (see, e.g., \cite{schuld2021machine, simeone2022introduction} for an introduction). Furthermore, we assume in this subsection that outputs of the model are obtained by averaging over an infinite number of shots, as in most of the literature on the subject (see, e.g., \cite{schuld2021machine}). 

A PQC encodes the classical input $x$ into a \emph{parameterized quantum embedding} defined by the state of an $n$-qubits state. The state is described by a $2^n\times 2^n$ density matrix $\rho(x|\theta)$, which is a positive semi-definite matrix with unitary trace, i.e., $\text{Tr}(\rho(x|\theta))=1$, where $\text{Tr}(\cdot)$ represents the trace operator. We write $N=2^n$ for the dimension of the Hilbert space on which density matrix $\rho(x|\theta)$ operates. The state $\rho(x|\theta)$ is obtained via the application of a parameterized unitary matrix $U(x|\theta)$ to a fiducial state $|0\rangle$ for the register of $n$ qubits, yielding \begin{align}\rho(x|\theta)=U(x|\theta)|0\rangle \langle 0| U(x|\theta)^\dagger,\label{eq:quantum_embedding}\end{align} where $\dagger$ represents the complex conjugate transpose operation.

Deterministic predictors can be in principle implemented via a PQC by considering the expected value of some \emph{observable} $O$ as the output of the model. An observable is defined by an $N\times N$ Hermitian matrix $O$. By the spectral theorem, an observable can be hence expressed in terms of its eigendecomposition (see, e.g., \cite[Sec. 5]{simeone2022introduction})
\begin{align}\label{eq:observable} O= \sum_{j=1}^{N'} o_j \Pi_j \end{align} with real eigenvalues $\{o_j\}_{j=1}^{N'}$ and projection matrices $\{ \Pi_j \}_{j=1}^{N'}$ satisfying the resolution-of-identity equality $\sum_{j=1}^{N'}\Pi_j = I$, where $N' \leq N$ is the number of distinct eigenvalues of the observable $O$. 

Accordingly, for a scalar target variable, the deterministic predictor is given by the expectation \begin{align}
   \label{eq:deterministic_output_pqc}
    \hat{y} = \text{Tr}(O \rho(x|\theta))=\langle O  \rangle_{\rho(x|\theta)}.
\end{align}
Note that multi-dimensional target spaces $\mathcal{Y}$ can be handled by considering a number of observables \cite{caro2022generalization}.  Henceforth, we will assume a scalar target variable $y \in \mathbb{R}$. Furthermore, we will assume that the discrete output space of the PQC $\hat{\mathcal{Y}}=\{o_j\}_{j=1}^{N'}$ is included in the target space $\mathcal{Y}$, i.e., $\hat{\mathcal{Y}} \subseteq \mathcal{Y}$. These assumptions are made to simplify the presentation, and they can be alleviated at the cost of a more cumbersome notation. 

Given the deterministic parametric predictor  \eqref{eq:deterministic_output_pqc}, training can be carried out based on training set $\mathcal{D}^\mathrm{tr}$ using local or global optimization schemes \cite{duffield2022bayesian, mitarai2018quantum, schuld2019evaluating, lavrijsen2020classical, rad2022surviving}, producing a trained parameter vector $\theta_{\mathcal{D}^\mathrm{tr}}$. Given the trained model $\text{Tr}(O \rho(x|\theta_{\mathcal{D}^\mathrm{tr}}))$, one can directly apply CP as described in the previous subsection in order to obtain well-calibrated set predictors. 

This direct application of CP to quantum machine learning has the important limitation of relying on the assumption that the expected value \eqref{eq:deterministic_output_pqc} can be evaluated exactly. In fact, in practice, the expectation in \eqref{eq:deterministic_output_pqc} can only be estimated based on a finite number of measurements, or shots, obtained by running the PQC multiple times and applying the projective measurement defined by projectors $\{ \Pi_j \}_{j=1}^{N'}$ to the quantum embedding $\rho(x|\theta)$. 


==> Sections/3_PCP.tex <==

\section{Conformal Prediction for Classical Probabilistic Models}
\label{sec:probabilistic_CP}

This section reviews the PCP approach introduced in \cite{wang2022probabilistic}, which is a variant of CP that applies post-hoc calibration to samples produced by a \emph{classical} probabilistic model.

Consider a parametric probabilistic predictor defined by a conditional distribution  $p(y|x,\theta)$ of target output $\mathbf{y}$ given input $\mathbf{x}=x$. For example, in regression, the distribution $p(y|x,\theta)$ may describe a Gaussian random variable $\mathbf{y}$ with mean and covariance dependent on input $x$ and parameter vector $\theta$; or it may describe a categorical random variable $\mathbf{y}$ with logit vector dependent on input $x$ and parameter vector $\theta$. The mentioned functions are typically implemented as neural networks with weight vector $\theta$ and input $x$. Model $p(y|x,\theta)$ can be trained using standard tools from machine learning, yielding a trained model parameter vector $\theta_{\mathcal{D}^\text{tr}}$ \cite{simeone2022introduction, shalev2014understanding}. 

PCP constructs a set predictor not directly as a function of the likelihood $p(y|x,\theta_{\mathcal{D}^\text{tr}})$ of the trained model, but rather as a function of a number of random predictions $\hat{\mathbf{y}}$ generated from the model $p(y|x,\theta_{\mathcal{D}^\text{tr}})$. As mentioned in Sec.~\ref{sec:intro}, the motivation of PCP is to obtain more flexible set predictors that can describe disjoint error bars \cite[Fig. 1]{wang2022probabilistic}. An illustration of PCP can be found in  Fig.~\ref{fig:pcp_scoring}. 

To elaborate, given test input $x$ and trained model $p(y|x,\theta_{\mathcal{D}^\text{tr}})$, PCP generates $M$ i.i.d. predictions $\hat{\mathbf{y}}^{1:M} = \{ \hat{\mathbf{y}}^m \}_{m=1}^M$, with each sample drawn from the model as
\begin{align}
    \label{eq:sampling_classical}
    \hat{\mathbf{y}}^m \sim p(y|x,\theta_{\mathcal{D}^\text{tr}}). 
\end{align} It then calibrates these predictions by using the calibration set. To this end, given the calibration set $\mathcal{D}^\text{cal}$, in an \emph{offline} phase, for each calibration example $z[i]\in \mathcal{D}^\text{cal}$, PCP generates $M$ i.i.d. random predictions $\hat{\mathbf{y}}^{1:M}[i] = \{ \hat{\mathbf{y}}^m[i] \}_{m=1}^M$, with each sample obtained from the model as $\hat{\mathbf{y}}^m[i]\sim p(y|x[i],\theta_{\mathcal{D}^\text{tr}})$. 

\begin{figure*}
\centering
\includegraphics[width=0.88\textwidth]{Figs/pcp_scoring.png}
\caption{ (\emph{i}) In PCP, the score for each calibration example $z[i]=(x[i],y[i])$ is evaluated based on independent random predictions $\hat{\mathbf{y}}^{1:M}[i]$ produced by the trained model as in  \eqref{eq:sampling_classical}. As an example, using the scoring function (\ref{eq:scoring_pcp}), the score is obtained by evaluating the  minimum distance between the true output $y[i]$ and the $M$ random predictions $\hat{\mathbf{y}}^m[i]$.  (\emph{ii}) The PCP set predictor uses the $M$ random predictions $\hat{\mathbf{y}}^{1:M}$ for test input $x$ in a similar way in order to evaluate the score of every possible candidate output $y'\in\mathcal{Y}$. With the scoring function (\ref{eq:scoring_pcp}), PCP yields a predictive set given by disjoint regions in the plane. This set is guaranteed to contain the true output $\mathbf{y}$ with the predetermined coverage level $1-\alpha$.}
  \label{fig:pcp_scoring}
\end{figure*}

Like CP, PCP also relies on the use of a  scoring function that evaluates the loss of the trained model on each data point. Unlike CP, the scoring function of PCP is not a function of a single, deterministic, prediction $\hat{y}$, but rather of the $M$ random predictions $\hat{\mathbf{y}}^{1:M}$ generated i.i.d. from the model $p(y|x,\theta_{\mathcal{D}^\text{tr}})$ for the given test input $x$. Accordingly, we write as $s((x,y)|\hat{\mathbf{y}}^{1:M})$ the scoring function, which measures the loss obtained by the trained model on an example $z=(x,y)$ based on the random predictions $\hat{\mathbf{y}}^{1:M}$. 

The work \cite{wang2022probabilistic} proposed the scoring function
\begin{align}
    \label{eq:scoring_pcp}
    s(z=(x,y)|\hat{\mathbf{y}}^{1:M}) = \min_{m \in \{1,...,M\}}| y - \hat{\mathbf{y}}^m|.
\end{align}This loss metric uses the best among the $M$ random predictions $\hat{\mathbf{y}}^m$ to evaluate the score on example $z$ as  the Euclidean distance $| y - \hat{\mathbf{y}}^m |$ between the best prediction $\hat{\mathbf{y}}^m$ and the output $y$ \cite{wang2022probabilistic}.

Having defined the scoring function as in  \eqref{eq:scoring_pcp}, PCP obtains a set predictor \eqref{eq:classical_CP_set_predictor} as for CP by replacing the scoring function  $s(z|\theta)$, e.g., the quadratic loss $(y-f(x|\theta))^2$, with the scoring function \eqref{eq:scoring_pcp} for both test and calibration pairs. This yields the set predictor
\begin{align}
\label{eq:prob_CP_set_predictor}
\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) &=\Big\{ y' \in \mathcal{Y} \hspace{-0.1cm}\: : \hspace{-0.1cm}\: {s}((x,y')|\hat{\mathbf{y}}^{1:M})  \:\leq\:  Q_{1-\alpha} \Big(\big\{ {s}( z[i]|\hat{\mathbf{y}}^{1:M}[i]  )\big\}_{i=1}^{ |\mathcal{D}^\text{cal}| } \Big)\Big\}.   
 \end{align} When evaluated using the scoring function (\ref{eq:scoring_pcp}), this results in a generally disjoint set of intervals for scalar variables (and circles for two-dimensional variables) \cite{wang2022probabilistic}.

As long as the examples in the calibration set $\mathbfcal{D}^\text{cal}$ and the test example $\mathbf{z}$ are finitely exchangeable random variables (Assumption~\ref{assum:classical}), the PCP set predictor \eqref{eq:prob_CP_set_predictor} is well calibrated as formalized next. 

\begin{theorem}[Calibration of PCP \cite{wang2022probabilistic}]\label{ther:pcp} Under Assumption~\ref{assum:classical} with sampling procedure following \eqref{eq:sampling_classical}, for any miscoverage level $\alpha \in (0,1)$ and for any trained model $\theta_{\mathcal{D}^{\text{tr}}}$, the PCP set predictor \eqref{eq:prob_CP_set_predictor} satisfies the inequality \begin{align}
    \label{eq:validity_pcp}
    \Pr( \mathbf{y} \in \mathbf{\Gamma}_M(\mathbf{x}|\mathbfcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) ) \geq 1-\alpha,
\end{align}with probability taken over the joint distribution of the test data $\mathbf{z}$, of the calibration data set $\mathbfcal{D}^\text{cal}$, and also over the independent random predictions $\hat{\mathbf{y}}^{1:M}$ and $\{\hat{\mathbf{y}}^{1:M}[i]\}_{i=1}^{|\mathcal{D}^\text{cal}|}$ produced by the model for test and calibration points.
\end{theorem}
A proof of Theorem~\ref{ther:pcp} is provided for completeness in Appendix~\ref{appendix:proofs}.



==> Sections/4_QCP.tex <==
\section{Quantum Conformal Prediction}
\label{sec:QCP}

In this section, we describe the proposed QCP method, a post-hoc calibration scheme for quantum machine learning that treats PQCs as implicit, i.e., likelihood-free, probabilistic models.  

\subsection{PQCs as Implicit Probabilistic Models}
\label{subsec:pqcs_as_implicit_prob_model}
As discussed in Sec.~\ref{subsec:quantum_models}, the output of PQCs is typically taken to be the expectation \eqref{eq:deterministic_output_pqc} of one or more observables. However, the exact evaluation of this quantity requires the capacity to run the PQC for an arbitrarily large number of times in order to average over a, theoretically infinite, number of shots. In contrast, in this section, we view the output of the PQC over any, potentially small, number of shots as probabilistic. 


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{Figs/cartoon_qcp.png}
  \caption{Illustration of QCP for a PQC with trained parameter vector  $\theta_{\mathcal{D}^\text{tr}}$ and for a scoring function $s((x,y)|\hat{\mathbf{y}}^{1:M})$ (see Sec.~\ref{subsubsec:quantum_scoring}): In the \emph{offline phase}, (\emph{i}) QCP first computes a score for each calibration example based on  $M$ random predictions produced by the PQC; (\emph{ii}) then, based on the  obtained $|\mathcal{D}^\text{cal}|$ calibration scores, QCP divides the real line into an acceptance region and a rejection region by using as a threshold the $(1-\alpha)$-quantile of the calibration scores. In the \emph{testing} phase,  (\emph{iii}) QCP constructs a set predictor for a test input $x$ by including in the set all  candidate outputs $y' \in \mathcal{Y}$ whose scores lie in the acceptance region.  (\emph{iv}) The obtained QCP set predictor (green circle) is guaranteed to satisfy the validity condition \eqref{eq:validity_qcp}.}
  \label{fig:QCP_cartoon}
\end{figure*}


To elaborate, let us fix a trained model parameter vector $\theta_{\mathcal{D}^\text{tr}}$, as well as a projective measurement defined by the projection matrices $\{\Pi_j\}_{j=1}^{N'}$ and corresponding numerical outputs $\{o_j\}_{j=1}^{N'}$ as in \eqref{eq:observable}. For any input $x$, the output $\hat{\mathbf{y}}$ obtained from the model equals value $o_j$ with probability \begin{align}
    \label{eq:single_measurement_distribution}
     p(\hat{\mathbf{y}}=o_j|x,\theta_{\mathcal{D}^\text{tr}})=\text{Tr}(\Pi_j \rho(x|\theta_{\mathcal{D}^\text{tr}})).
\end{align} 
The distribution  \eqref{eq:single_measurement_distribution} is generally not directly accessible. Rather, the model is implicit, in the sense that all that can be observed by a user are samples $\hat{\mathbf{y}}\sim  p(y|x,\theta_{\mathcal{D}^\text{tr}})$ drawn from it.

Treating a PQC as an implicit probabilistic model has the additional advantage that one can seamlessly account for the presence of \emph{quantum hardware noise}. To this end, let us write as $\tilde{\rho}(x|\theta_{\mathcal{D}^\text{tr}})$ the quantum embedding produced by a noisy quantum computer. The density matrix $\tilde{\rho}(x|\theta_{\mathcal{D}^\text{tr}})$ accounts also for the effect of quantum channels describing gate noise \cite{knill2005quantum, harrow2003robustness, sharma2020noise, he2020zero}. Then, the noisy PQC can be viewed as an implicit probabilistic model that, for any input $x$,   produces a sample $\hat{\mathbf{y}}$ equal to $o_j$ with probability\begin{align}
    \label{eq:single_measurement_distribution_noisy}
     p(\hat{\mathbf{y}}=o_j|x,\theta_{\mathcal{D}^\text{tr}})=\text{Tr}(\Pi_j \tilde{\rho}(x|\theta_{\mathcal{D}^\text{tr}}))
\end{align} for all $j=1,...,N'$. One can also similarly account for other sources of noise, including in the preparation and measurement phases \cite{chow2010detecting, bravyi2021mitigating, van2022model}. 

We will follow the standard assumption that each new $m$-th measurement, or shot, for a given input $x$ produces an independent output $\hat{\mathbf{y}}^{m}$ with distribution \eqref{eq:single_measurement_distribution_noisy}. Accordingly, given an input $x$, we will assume the availability of  $M$ independent measurements $\hat{\mathbf{y}}^{1:M} = \{ \hat{\mathbf{y}}^m \}_{m=1}^M$ from distribution (\ref{eq:single_measurement_distribution_noisy}).  This is in line with the assumption made in PCP, which considers the output predictions in (\ref{eq:sampling_classical}) to be i.i.d. While we will not elaborate on this point further, we note that it is also possible to extend the properties of QCP to more general measurement models characterized by correlation across the measurement outputs $\hat{\mathbf{y}}^{1:M}$ produced for each input $x$, as long as there is no correlation across shots for distinct inputs $x$. This correlation may arise, for instance, due to a  system or diffusive drift in the quantum noise processes \cite{schwarz2011detecting}. {\color{black} We note that, in practice, correlations may also extend across multiple inputs $x$ \cite{deville2021new}. }





\subsection{Quantum Conformal Prediction}
For a test input $x$, QCP processes the $M$ predictions $\hat{\mathbf{y}}^{1:M}=\{ \hat{\mathbf{y}}^m \}_{m=1}^M$ made via the PQC with the goal of producing a well-calibrated set predictor with generalization guarantees. As detailed in the previous subsection, the $M$ predictions are obtained via $M$ independent measurements of the output of the PQC, which are distributed as in \eqref{eq:single_measurement_distribution_noisy}. Following the CP framework, QCP leverages a calibration data set $\mathcal{D}^\text{cal}$ consisting  of $|\mathcal{D}^\text{cal}|$ calibration examples $z[i]$ for $i=1,...,|\mathcal{D}^\text{cal}|$. In the rest of this subsection, we detail the operation of QCP, which is illustrated in Fig. \ref{fig:QCP_cartoon} and summarized in Algorithm \ref{alg:QCP}. 

Like CP and PCP, QCP is divided into an offline phase, taking place only once based on the calibration data set, and a testing phase in which set predictions are produced for a set of desired test inputs. Both phases rely on the specification of a \emph{scoring function} $s(z|{\hat{\mathbf{y}}^{1:M}})$, which, given an example $z=(x,y)$,  quantifies the prediction loss associated with samples $\hat{\mathbf{y}}^{1:M}$ produced by the PQC in response to an input $x$ when the correct output is $y$. The scoring function may be selected as in (\ref{eq:scoring_pcp}), as suggested in \cite{wang2022probabilistic}. More general choices, which will be proved to be advantageous in Sec.~\ref{sec:experimental_results}, are presented in Sec.~\ref{subsubsec:quantum_scoring}.

During the \emph{offline phase}, for each calibration point $z[i]$,  the PQC  with trained model parameter vector $\theta_{\mathcal{D}^\text{tr}}$ generates $M$ independent predictions $\hat{\mathbf{y}}^{1:M}[i]=\{ \hat{\mathbf{y}}^m[i] \}_{i=1}^M$ from distribution \eqref{eq:single_measurement_distribution} (Fig.~\ref{fig:QCP_cartoon}-(\emph{i})).  Then, following the CP methodology detailed in Sec.~\ref{sec:classical_CP_procedure},  QCP divides the possible values returned by the scoring function into an \emph{acceptance region} and a \emph{rejection region} (Fig.~\ref{fig:QCP_cartoon}-(\emph{ii})). The acceptance threshold is given by  the $\lceil(1-\alpha)(|\mathcal{D}^\text{cal}|+1)\rceil$-th smallest value in the set $\{ s(z[1]|\hat{\mathbf{y}}^{1:M}[1])  ,...,s(z[|\mathcal{D}^\text{cal}|]|\hat{\mathbf{y}}^{1:M}[|\mathcal{D}^\text{cal}|]),\infty \}$ of scores for the calibration data points. As in Sec.~\ref{sec:classical_CP_procedure}, this quantity is denoted as $Q_{1-\alpha}( \{  s(z[i]|\hat{\mathbf{y}}^{1:M}[i])  \}_{i=1}^{|\mathcal{D}^\text{cal}|} )$.


In the \emph{testing phase}, for a test input $x$, the PQC with the same trained model parameter vector $\theta_{\mathcal{D}^\text{tr}}$ produces $M$ predictions $\hat{\mathbf{y}}^{1:M}$ (Fig.~\ref{fig:QCP_cartoon}-(\emph{iii}, dotted box)). Finally, QCP produces the prediction set $\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) \subseteq \mathcal{Y}$ of the \emph{target space} $\mathcal{Y}$, by including in the set predictor $\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}})$ all candidate outputs $y' \in \mathcal{Y}$ whose scores $s((x,y')|\hat{\mathbf{y}}^{1:M})$ lie in the acceptance region (Fig.~\ref{fig:QCP_cartoon}-(\emph{iii})). Accordingly, the QCP set predictor is defined as
\begin{align}
\label{eq:quantum_CP_set_predictor}
\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) &=\Big\{ y' \in \mathcal{Y} \hspace{-0.1cm}\: : \hspace{-0.1cm}\: {s}((x,y')|\hat{\mathbf{y}}^{1:M})  \:\leq\:  Q_{1-\alpha} \Big(\big\{ {s}( z[i]|\hat{\mathbf{y}}^{1:M}[i]   )\big\}_{i=1}^{ |\mathcal{D}^\text{cal}| } \Big)\Big\}.   
\end{align}

In Algorithm \ref{alg:QCP}, which summarizes QCP, the complexity of the offline phase  (lines 3--7) can be amortized by reusing the threshold identified during this phase across multiple test inputs. In this regard, for general scoring functions, it may not be feasible to try out all values of $y'\in\mathcal{Y}$ for inclusion in the predictive set (lines 11--14). This problem can be addressed in one of two ways. First, for specific scoring functions,  such as \eqref{eq:scoring_pcp}, the predictive set can be obtained in closed form, as we elaborate on in Sec.~\ref{subsubsec:quantum_scoring}. Second, it is possible to quantize the target space in order to reduce the complexity of the search among values of $y'\in\mathcal{Y}$ to include in the predictive set  \cite{chen2018discretized}. 

\begin{algorithm}[hbt!] %!
\DontPrintSemicolon
\LinesNumbered
\smallskip
\KwIn{trained parameter vector $\theta_{\mathcal{D}^\text{tr}}$ for the PQC; calibration data set $\mathcal{D}^\text{cal}=\{ z[i]=(x[i],y[i]) \}_{i=1}^{|\mathcal{D}^\text{cal}|}$; test input $x$; number of shots $M\geq 1$; desired coverage level $1-\alpha$}
\KwOut{well-calibrated predictive set $\Gamma_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}})$ at coverage level $1-\alpha$  }
\vspace{0.15cm}
\hrule
\vspace{0.15cm}
{\bf choose}  scoring function $s( (x,y)|\hat{\mathbf{y}}^{1:M})$ as outlined  in Sec.~\ref{subsubsec:quantum_scoring}\\
\texttt{Offline phase}\\
\For{{\em $i$-th calibration data example $z[i]$ with $i=1,...,|\mathcal{D}^\text{cal}|$ }}{\vspace{0.1cm}
given input $x[i]$, produce $M$ independent predictions $\hat{\mathbf{y}}^{1:M}[i]=\{ \hat{\mathbf{y}}^{m}[i] \}_{m=1}^{M}$ via $M$ shots of the PQC \\
compute the corresponding score $s(z[i]|\hat{\mathbf{y}}^{1:M}[i])$
}
find the  $\lceil(1-\alpha)(|\mathcal{D}^\text{cal}|+1)\rceil$-th smallest value among the obtained scores, which is denoted as $Q_{1-\alpha}( \{  s(z[i]|\hat{\mathbf{y}}^{1:M}[i])  \}_{i=1}^{|\mathcal{D}^\text{cal}|} )$ \\
\texttt{Testing phase for input $x$}\\
{\bf initialize} predictive set $\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) \leftarrow \{ \}$\\
for test input $x$, make $M$ predictions $\hat{\mathbf{y}}^{1:M}=\{ \hat{\mathbf{y}}^{m} \}_{m=1}^{M}$ via PQC  \\
\For{{\em candidate output $y' \in \mathcal{Y}$}}{\vspace{0.1cm}
compute the corresponding score $s((x,y')|\hat{\mathbf{y}}^{1:M})$\\
\hspace{-0.25cm}\uIf{ ${s}((x,y')|\hat{\mathbf{y}}^{1:M})  \:\leq\:  Q_{1-\alpha}( \{  s(z[i]|\hat{\mathbf{y}}^{1:M}[i])  \}_{i=1}^{|\mathcal{D}^\text{cal}|} )$}{
$\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) \leftarrow \mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}})  \cup \{ y' \}$
  }
}
{\bf return} the predictive set $\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}})$ for test input $x$
\caption{Quantum Conformal Prediction (QCP)}
\label{alg:QCP}
\end{algorithm}



\subsection{Theoretical Calibration Guarantees}
\label{subsubsec:qcp_theoretical}

QCP inherits the calibration properties of CP and PCP. In particular, as long as the examples in the calibration set $\mathbfcal{D}^\text{cal}$ and the test example $\mathbf{z}$ are finitely exchangeable random variables (Assumption~\ref{assum:classical}),  the QCP set predictor \eqref{eq:quantum_CP_set_predictor} is well calibrated at coverage level $1-\alpha$, as detailed next. 

\begin{theorem}[Calibration of QCP]\label{ther:qcp} Under Assumption~\ref{assum:classical} with  sampling procedure following \eqref{eq:single_measurement_distribution_noisy}, for any coverage level $1-\alpha \in (0,1)$ and for any trained PQC with model parameter vector $\theta_{\mathcal{D}^{\text{tr}}}$, the QCP set predictor \eqref{eq:prob_CP_set_predictor} satisfies the inequality \begin{align}
    \label{eq:validity_qcp}
    \Pr( \mathbf{y} \in \mathbf{\Gamma}_M(\mathbf{x}|\mathbfcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) ) \geq 1-\alpha,
\end{align}with probability taken over the joint distribution of the test data $\mathbf{z}$, of the calibration data set $\mathbfcal{D}^\text{cal}$, and of the independent random predictions $\hat{\mathbf{y}}^{1:M}$ and $\{\hat{\mathbf{y}}^{1:M}[i]\}_{i=1}^{|\mathcal{D}^\text{cal}|}$ produced by the PQC for test and calibration points, respectively.
\end{theorem}
A proof of Theorem~\ref{ther:qcp} is provided in Appendix~\ref{appendix:proofs}.


\subsection{Scoring Function}
\label{subsubsec:quantum_scoring}

In this subsection, we elaborate on possible choices for the scoring function to be used in QCP. We note that the same considerations apply also to PCP.  We start by interpreting the scoring function \eqref{eq:scoring_pcp}  assumed by PCP as the loss associated with a \emph{non-parametric estimate} of the conditional distribution $p(y|x,\theta)$ of the target variable $\mathbf{y}$ given the input variable $\mathbf{x}$, where the estimate is obtained based on the samples $\hat{\mathbf{y}}^{1:M}$ produced by the model. We then observe that any loss function for a probabilistic predictor, coupled with an estimate of the conditional distribution $p(y|x,\theta)$, yields a valid scoring function. 

To elaborate, we review the notion of loss function for an \emph{explicit} probabilistic predictor ${p}(y|x,\theta)$ (see, e.g., \cite[Sec. 2.2.2]{vovk2022algorithmic}). An explicit probabilistic predictor is one that outputs the probability distribution ${p}(y|x,\theta)$.  Given an example $z=(x,y)$, the loss accrued by probabilistic model $p(y|x,\theta)$ can be evaluated as $g(p(y|x,\theta))$, where $g(\cdot)$ is a strictly decreasing function. Accordingly, the loss increases if the model assigns a lower probability $p(y|x,\theta)$ to the correct output $y$ given input $x$.  Typical examples of such functions include the negative logarithm, which yields the \emph{log-loss} $-\log p(y|x,\theta)$, and the \emph{inverse function} $1/p(y|x,\theta)$ (see, e.g., \cite[Sec. 6.7]{simeone2022introduction} for further examples). 

The class of loss functions outlined in the previous paragraph is not applicable to implicit models, which do not produce the probabilities $p(y|x,\theta)$, but only samples from this distribution. However, given $M$ samples $\hat{\mathbf{y}}^{1:M}$ generated i.i.d. from the distribution $p(y|x,\theta)$, one can obtain an estimate $\hat{p}(y|x,\theta)$ of  the probability $p(y|x,\theta)$. The key observation of this subsection is that such an estimate can be used to define a scoring function as follows.

\begin{definition}[Scoring function for implicit models]\label{def:scoring}
Given $M$ i.i.d. predictions $\hat{\mathbf{y}}^{1:M}$  drawn from a model $p(y|x,\theta)$ for input $x$, a scoring function for input-output pair $z=(x,y)$ is defined as
\begin{align}\label{eq:newscore}
    s(z|\hat{\mathbf{y}}^{1:M}) = g(\hat{p}(y|x,\theta)),
\end{align}
where $g(\cdot)$ is a monotonically decreasing function and $\hat{p}(y|x,\theta)$ is an estimator of the probability $p(y|x,\theta)$ obtained as a function of the samples $\hat{\mathbf{y}}^{1:M}$.
\end{definition}

\begin{figure*}
\centering
\includegraphics[width=0.88\textwidth]{Figs/qcp_scoring.png}
\caption{ {\color{black}(\emph{i}) In QCP, the score for each calibration example $z[i]=(x[i],y[i])$ is evaluated based on independent random predictions $\hat{\mathbf{y}}^{1:M}[i]$ produced by the trained model as in  \eqref{eq:sampling_classical}. Using the proposed scoring function \eqref{eq:newscore}-\eqref{eq:non_para_conditional_est}, the score is obtained by evaluating the $k$-th smallest distance between the true output $y[i]$ and the $M$ random predictions $\hat{\mathbf{y}}^m[i]$.  (\emph{ii}) The QCP set predictor uses the $M$ random predictions $\hat{\mathbf{y}}^{1:M}$ for test input $x$ in order to evaluate the score of every possible candidate output $y'\in\mathcal{Y}$. QCP yields a predictive set given by disjoint regions in the plane. By not relying solely on the closest prediction as PCP (see Fig.~\ref{fig:pcp_scoring}), the prediction sets produced by QCP can be more robust to noisy predictions (see Sec.~\ref{sec:experimental_results}). This set is guaranteed to contain the true output $\mathbf{y}$ with the predetermined coverage level $1-\alpha$.}}
  \label{fig:qcp_scoring}
\end{figure*}


To define a score function as in (\ref{eq:newscore}) one can generally use either  \emph{non-parametric} density estimators, including kernel density estimation \cite{parzen1962estimation}, variable kernel density estimation \cite{terrell1992variable, loftsgaarden1965nonparametric}, and histogram-based density estimation \cite{bishop2006pattern}; or \emph{parametric} density estimators, including contrastive density learning \cite{gutmann2012noise}, and normalizing flows \cite{papamakarios2021normalizing} (see, e.g., \cite[Sec.~7.3]{simeone2022machine} for a summary). 

We elaborate here on the use of non-parametric estimators, and we focus as done throughout the article on a scalar target variable $y$.  Given $M$ samples $\hat{\mathbf{y}}^{1:M}$ drawn i.i.d. from distribution $p(y|x,\theta)$, and a positive integer $k\leq M$, the \emph{$k$-nearest neighbor ($k$-NN) density estimator} of $p(y|x,\theta)$ is given by \cite{loftsgaarden1965nonparametric}
\begin{align}
     \label{eq:non_para_conditional_est}
     \hat{p}(y|x,\theta) = \frac{k}{2M | y - \hat{\mathbf{y}}^m|_{(k)}},
 \end{align}
where $| y - \hat{\mathbf{y}}^m|_{(k)}$ is the $k$-th smallest Euclidean distance in the set of distances $\{| y - \hat{\mathbf{y}}^m|\}_{m=1}^{M}$. This estimate is asymptotically consistent:  As long as $k$ grows suitably with $M$, the estimate \eqref{eq:non_para_conditional_est} tends to the true distribution $p(y|x,\theta)$  pointwise  in probability \cite{loftsgaarden1965nonparametric}.  In particular, parameter $k$ should be selected in such a way that the limits $\lim_{M \rightarrow \infty}k(M)=\infty$ and $\lim_{M \rightarrow \infty}k(M)/M=0$ are satisfied. An example of such dependence is given by \cite{loftsgaarden1965nonparametric}
\begin{align} \label{eq:qcp_scoring_consistent}
    k(M) = \big\lceil M^{1/2} \big\rceil.
\end{align}


With this background in place, we can now show that the PCP scoring function \eqref{eq:scoring_pcp} corresponds to a special case of the class of scoring functions (\ref{eq:newscore}). In fact, with the inverse function for $g(\cdot)$ and the $1$-NN estimator \eqref{eq:non_para_conditional_est}, the scoring function (\ref{eq:newscore}) reads \begin{align}
    \label{eq:pcp_scoring_from_generalized}
    s(z=(x,y)|\hat{\mathbf{y}}^{1:M}) &= \frac{1}{\hat{p}(y|x,\theta)} \nonumber \\&= 2M | y-\hat{\mathbf{y}}^m|_{(1)},
\end{align}which equals \eqref{eq:scoring_pcp}  apart from an inessential multiplicative constant. 

In the experiments in Sec.~\ref{sec:experimental_results}, we will consider the more general scoring function in class \eqref{eq:pcp_scoring_from_generalized} obtained with the $k$-NN predictor \eqref{eq:non_para_conditional_est}. With this choice, the QCP set predictor \eqref{eq:quantum_CP_set_predictor}, as well as the PCP set predictor \eqref{eq:prob_CP_set_predictor} can be expressed as 
\begin{align}
\label{eq:closed_form_genreal_scoring_pcp_and_qcp}
&\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}}) =\Big\{ y' \in \mathcal{Y} \hspace{-0.1cm}\: : \hspace{-0.1cm}\: \sum_{m=1}^M \mathbbm{1}\big(y' \in B_{q(\mathcal{D}^\text{cal})}(\hat{\mathbf{y}}^m)\big) \geq k \}\Big\},
 \end{align}
in which $B_{q(\mathcal{D}^\text{cal})}(y)$ is the closed interval with center point $y$, i.e., $B_r(y) = \{ y' \in \mathcal{Y}: | y - y'| \leq r \}$, and radius $q(\mathcal{D}^\text{cal})=  Q_{1-\alpha} \big(\big\{ 
| y[i] - \hat{\mathbf{y}}^m[i] |_{(k)}
\big\}_{i=1}^{ |\mathcal{D}^\text{cal}| } \big)$. {\color{black} Illustration of the QCP set predictor with $k$ chosen as \eqref{eq:qcp_scoring_consistent} can be found in Fig.~\ref{fig:qcp_scoring}, while experimental study regarding the impact of $k$ on the size of the set predictor \eqref{eq:closed_form_genreal_scoring_pcp_and_qcp} can be found in Appendix~\ref{appendix:additional_experiments}. }



{\color{black}
\subsection{Application to Quantum Data} \label{sec:application_to_quantum}
So far we have focused on situations in which input data $x$ is of classical nature. Accordingly, given a pre-trained PQC, one can produce $M$ copies of the quantum embedding state $\rho(x|\theta_{\mathcal{D}^\text{tr}})$ to be used by QCP in order to yield the set predictor $\mathbf{\Gamma}_M(x|\mathcal{D}^\text{cal},\theta_{\mathcal{D}^\text{tr}})$. However, QCP can be equally well applied to settings in which the pre-trained model takes as input quantum data. We briefly elaborate on this applications in the rest of this subsection by focusing on the classification of quantum data. 

    Assume that there are $C$ classes of quantum states, indexed by variable $y \in \{1,...,C\}$, such that the $y$-th class corresponds to a density matrix $\rho(y)$. The data generating mechanism is specified by a distribution $p(y)$ over the class index $y$ and by the set of density matrices $\rho(y)$ with $y\in \{1,...,C\}$. Given any pre-designed positive operator-valued measurement (POVM) defined by positive semidefinite matrices $\mathcal{P}=\{\mathrm{P}_1,...,\mathrm{P}_C\}$,  the POVM produces output $\hat{\mathbf{y}}$ with probability  \begin{align} \label{eq:pred_single_main}
    \hat{\mathbf{y}} \sim p(y|\rho, \mathcal{P})= \text{Tr}(\mathrm{P}_y \rho ).
    \end{align}
    Note that the POVM $\mathcal{P}$ can be implemented via a pre-trained PQC with parameter vector $\theta_{\mathcal{D}^\text{tr}}$ followed by a projective measurement as per the setting considered above, yielding \eqref{eq:single_measurement_distribution} when removing input $x$.  Here we adopt a more general formulation. As we will see in Sec.~\ref{sec:exp_qc}, this allows us to consider other quantum detectors such as pretty good measurements \cite{hausladen1994pretty, gambs2008quantum}.

    The goal of QCP is to use the predesigned model operating on $M$ copies of a test state $\rho \in \{\rho(1),...,\rho(C)\}$, denoted as $\rho^{\otimes M}$, as well as $M$ copies of each example in the calibration data set $\mathcal{D}^\text{cal}$, to produce a set predictor $\mathbf{\Gamma}_M(\rho^{\otimes M}|\mathcal{D}^\text{cal},\mathcal{P})$ that contains the true label with predetermined coverage level $1-\alpha$. The calibration data is of the form $\mathcal{D}^\text{cal}=\{(\rho(y[i])^{\otimes M},y[i])\}_{i=1}^{|\mathcal{D}^\text{cal}|}$, where label  $y[i]\in \{1,...,C\}$ and $M$ copies of corresponding state $\rho(y[i])$ are available for each $i$-th calibration example. Mathematically, the reliability requirement can be expressed as the inequality \begin{align}
        \label{eq:qcp_QC_main}
        \Pr\big(\mathbf{y} \in \mathbf{\Gamma}_M(\rho(\mathbf{y})^{\otimes M}|\mathbfcal{D}^\text{cal},\mathcal{P})\big) \geq 1-\alpha,
    \end{align}
    where the probability $\Pr(\cdot)$ is taken over the i.i.d. calibration and test labels $\mathbf{y}, \mathbf{y}[1],...,\mathbf{y}[|\mathcal{D}^\text{cal}|]\sim p(y)$  and over the independent random predictions $\hat{\mathbf{y}}^{1:M}$ and $\{\hat{\mathbf{y}}^{1:M}[i]\}_{i=1}^{|\mathcal{D}^\text{cal}|}$ in \eqref{eq:pred_single_main}.

    QCP can be directly applied to the test predictions $\hat{\mathbf{y}}^{1:M}$ and to the calibration predictions $\{\hat{\mathbf{y}}^{1:M}[i]\}_{i=1}^{|\mathcal{D}^\text{cal}|}$ as detailed in Algorithm 1. By Theorem 3, QCP satisfies the reliability condition \eqref{eq:validity_qcp}. We also emphasize, following the discussions in Sec. IV-A, that the result applies also in the presence of quantum noise affecting the copies of the input states. Such noise can be generally expressed as a channel $\mathcal{N}(\cdot)$ acting on the $M$ copies as $\mathcal{N}(\rho^{\otimes M})$, as long as the same channel $\mathcal{N}(\cdot)$ affects both test and calibration input examples.}

==> Sections/5_finite_number_guarantee.tex <==
\section{Calibration Guarantees over a Finite Number of Experiments}
\label{sec:finite_number_guarantee}
In the previous sections, we have described CP schemes that satisfy calibration conditions, namely \eqref{eq:validity}, \eqref{eq:validity_pcp}, and \eqref{eq:validity_qcp}, that are defined on average over the calibration and test data points. For PCP and QCP, the average is also taken with respect to the random predictions produced for calibration and test data points. In this section, we elaborate on the practical significance of this expectation.



Suppose that we run CP, PCP or QCP (Algorithm~\ref{alg:QCP}) over $K$ runs that use independent calibration and test data. What is the fraction of such runs that  meet the condition that the true output is included in the predictive set? Ideally, this fraction will be close to the desired target $1-\alpha$ with high probability. In fact, by the results in the previous sections and by the law of large numbers, as $K$ grows large, this fraction of ``successful'' experiments will tend to $1-\alpha$. What can be guaranteed for a finite number $K$ of experiments? In the following, we address this question for conventional CP first, and then for PCP and QCP.

\subsection{Conventional CP}
Following the setting described above, let us consider $K$ experiments, such that in each $k$-th experiment we draw calibration and test data from the joint distribution $p(\mathcal{D}^\text{cal},z)$, i.e., $(\mathbfcal{D}^\text{cal}_k, \mathbf{z}_k) \sim p(\mathcal{D}^\text{cal},z)$. For each experiment, we evaluate whether the prediction set \eqref{eq:classical_CP_set_predictor} produced by CP contains the true target label $\mathbf{y}_k$ or not. Accordingly, the fraction of ``successful'' experiments is given by \begin{align}
    \label{eq:empirical_cov_dcp}
    \hat{\mathbf{P}}= \frac{1}{K}\sum_{k=1}^K \mathbbm{1}\big(\mathbf{y}_k \in \Gamma(\mathbf{x}_k|\mathbfcal{D}_k^\text{cal},\theta_{\mathcal{D}^\text{tr}})\big),
\end{align} where $\mathbbm{1}(\cdot)$ is the indicator function ($\mathbbm{1}(\text{true})=1$ and $\mathbbm{1}(\text{false})=0$). To restate the question posed at the beginning of this section, given $K$, how large can we guarantee the success rate $\hat{P}$ to be? 


By the exchangeability of calibration and test data (Assumption 1), which implies the exchangeability of the $|\mathcal{D}^\text{cal}|+1$ scores evaluated on calibration and test data (see Appendix~\ref{appendix:proofs}), the distribution of random variable $K\hat{\mathbf{P}}$ is given by the binomial
\begin{align}
    \label{eq:convergence_pmf}
    K\hat{\mathbf{P}} \sim \text{Binom}\bigg(K, \frac{\lceil (1-\alpha)(|\mathcal{D}^\text{cal}|+1) \rceil}{|\mathcal{D}^\text{cal}|+1}\bigg),
\end{align}
if ties between the $|\mathcal{D}^\text{cal}|+1$ scores occur with probability zero (see \cite{ lei2018distribution, tibshirani2019conformal} for other uses of this assumption). Note that  the distribution \eqref{eq:convergence_pmf} can be recovered from \cite[Sec.~C]{angelopoulos2021gentle} by setting the number of test points to be one (see also \cite{vovk2012conditional}).


This implies that the success rate $\hat{\mathbf{P}}$ is larger than $1-\alpha-\epsilon$ for any $\epsilon>0$ with probability \begin{align}
    \label{eq:convergence_theor}
    &\Pr(  \hat{\mathbf{P}} \geq 1-\alpha -\epsilon ) = I_{ \frac{\lceil (1-\alpha)(|\mathcal{D}^\text{cal}|+1) \rceil}{|\mathcal{D}^\text{cal}|+1}   } ( \lceil K(1-\alpha-\epsilon) \rceil, \lfloor K(\alpha+\epsilon)\rfloor+1 ),
\end{align}
with regularized incomplete beta function $I_x(a,b)=B(x;a,b)/B(a,b)$, where $B(x;a,b)=\int_{0}^x t^{a-1}(1-t)^{b-1}\mathrm{d}t$ and $B(a,b)=B(1;a,b)$ \cite{jowett1963relationship}.

Fig.~\ref{fig:convergence_cp_theory} shows the probability distribution of random variable $\hat{\mathbf{P}}$, as well as the probability (\ref{eq:convergence_theor})  as a function of tolerance level $\epsilon$ for different number of experiments $K=100,1000,10000$, given  $\alpha=0.1$ and $|\mathcal{D}^\text{cal}|=9$. The top figure confirms that, by the law of large numbers, the distribution of success rate $\hat{\mathbf{P}}$ concentrates around the value $1-\alpha=0.9$. The bottom figure can be used to identify a value of the \emph{backoff probability} $\epsilon$ that allows one to obtain finite-$K$ guarantees on the success rate $1-\alpha-\epsilon$. For instance,  when $K = 1000$, we observe that setting $\epsilon=0.03$ guarantees a success rate $\hat{\mathbf{P}}$ no smaller than $0.87$ with probability larger than $0.999$.


%For instance, {\color{red} in order to ensure the probability (\ref{eq:convergence_theor}) larger than $0.999$, we need backoff probability $\epsilon=0.1, 0.03, 0.01$ for $K=100,1000,10000$, respectively; while to ensure probability (\ref{eq:convergence_theor}) larger than $0.99$, we need $\epsilon=0.075, 0.023, 0.007$, for $K=100,1000,10000$, respectively.}



\begin{figure}
  \centering
  \includegraphics[width=0.48\textwidth]{Figs/convergence_theory.pdf}
  \caption{(top) Normalized density of the empirical coverage rate $\hat{\mathbf{P}}$ obtained from $K=100,1000,10000$ independent trials. (bottom) Probability that the empirical coverage rate $\hat{\mathbf{P}}$ satisfies the validity condition with tolerance level, or backoff probability, $\epsilon$ as a function of $\epsilon$, for $K=100,1000,10000$ independent trials  ($\alpha=0.1, |\mathcal{D}^\text{cal}|=9$).}
  \label{fig:convergence_cp_theory}
\end{figure}


\subsection{Probabilistic and Quantum CP}
In the case of PCP and QCP, each $k$-th experiment involves also the  predictions $\{\hat{\mathbf{y}}_k^{1:M}[i]\}_{i=1}^{|\mathcal{D}^\text{cal}|}$ for the calibration points $\mathbfcal{D}^\text{cal}_k$, and  $\hat{\mathbf{y}}_k^{1:M}$ for the test data $\mathbf{z}_k$, following either \eqref{eq:sampling_classical} (PCP) or \eqref{eq:single_measurement_distribution_noisy} (QCP). Despite the presence of the additional randomness due to the stochastic predictions, the finite-$K$ guarantees \eqref{eq:convergence_pmf}-\eqref{eq:convergence_theor} still hold for the fraction of ``successful'' experiments
\begin{align}
    \label{eq:empirical_cov_qcp}
    \hat{\mathbf{P}}_M := \frac{1}{K}\sum_{k=1}^K \mathbbm{1}\big(\mathbf{y}_k \in \mathbf{\Gamma}_M(\mathbf{x}_k|\mathbfcal{D}_k^\text{cal},\theta_{\mathcal{D}^\text{tr}})\big)
\end{align}
for PCP and QCP if ties between the $|\mathcal{D}^\text{cal}|+1$ scores occur with probability zero. This is because the $|\mathcal{D}^\text{cal}|+1$ scores for calibration and test data are exchangeable also for PCP and QCP due to the exchangeability of calibration and test data (Assumption~\ref{assum:classical}), and to the independence of $M$ predictions \eqref{eq:sampling_classical}, \eqref{eq:single_measurement_distribution_noisy} for distinct inputs. 


